$H^1$-norm stability and convergence of an L2-type method on nonuniform meshes for subdiffusion equation

This work establishes $H^1$-norm stability and convergence for an L2 method on general nonuniform meshes when applied to the subdiffusion equation. Under mild constraints on the time step ratio $\rho_k$, such as $0.4573328\leq \rho_k\leq 3.5615528$ for $k\geq 2$, the positive semidefiniteness of a crucial bilinear form associated with the L2 fractional-derivative operator is proved. This result enables us to derive long time $H^1$-stability of L2 schemes. These positive semidefiniteness and $H^1$-stability properties hold for standard graded meshes with grading parameter $1<r\leq 3.2016538$. In addition, error analysis in the $H^1$-norm for general nonuniform meshes is provided, and convergence of order $(5-\alpha)/2$ in $H^1$-norm is proved for modified graded meshes when $r>5/\alpha-1$. To the best of our knowledge, this study is the first work on $H^1$-norm stability and convergence of L2 methods on general nonuniform meshes for the subdiffusion equation.

==> tmp_L2nonuniform_siam_header.tex <==
\title{$H^1$-stability of an L2-type method on general nonuniform meshes for subdiffusion equation\thanks{Submitted in June 2022.}}

\author{
Chaoyu Quan
\thanks{SUSTech International Center for Mathematics, Southern University of Science and Technology, Shenzhen, P.R. China (\email{quancy@sustech.edu.cn}).}
\and
Xu Wu
\thanks{Department of Mathematics,  Harbin Institute of Technology, Harbin 150001, China; Department of Mathematics, Southern University of Science and Technology, Shenzhen, China (\email{11849596@mail.sustech.edu.cn}).}
}


% Custom SIAM macro to insert headers
\headers{$H^1$-stability of L2-type method}{C. Quan and X. Wu}

